Spatial Signatures of Electron Correlation in Least-Squares Tensor Hyper-Contraction

Least Squares Tensor Hypercontraction (LS-THC) has received some attention in recent years as an approach to reduce the significant computational costs of wavefunction based methods in quantum chemistry. However, previous work has demonstrated that the LS-THC factorization performs disproportionately worse in the description of wavefunction components (e.g. cluster amplitudes $\hat{T}_2$) than Hamiltonian components (e.g. electron repulsion integrals $(pq|rs)$). This work develops novel theoretical methods to study the source of these errors in the context of the real-space $\hat{T}_2$ kernel, and reports, for the first time, the existence of a "correlation feature" in the errors of the LS-THC representation of the "exchange-like" correlation energy $E_X$ and $\hat{T}_2$ that is remarkably consistent across ten molecular species, three correlated wavefunctions, and four basis sets. This correlation feature portends the existence of a "pair-point kernel" missing in the usual LS-THC representation of the wavefunction, which critically depends upon pairs of grid points situated close to atoms and with inter-pair distances between one and two Bohr radii. These findings point the way for future LS-THC developments to address these shortcomings.

==> src/todo.tex <==
\section{TODO}

ADD TODO ITEMS HERE.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% OLD OLD OLD
% RETAINING FOR SOME OF THE NUMBERS IN HERE, WILL DELETE LATER
\iffalse
New items are indicated in {\color{red} RED}. Mark which ones are in which state as you see them. Items in {\color{blue} BLUE} are things that we need to do with the final cleanup.

\begin{enumerate}
    \item{Add citations, or at least indicate where you think they should go [ONGOING]} 
    \item{Add nonumber command to align equations where we don't want numbering [ONGOING]}
    \item{Add LaTeX labels to all your equations.}
    \item{Can you give me an average and st. dev on the $R^2$ biexponential fits for the whole dataset in the single point grid section, along with the average ``turnover'' point for $E_C$ and $E_X$ where the contribution from the ``fast'' part of the biexponential is equal to the ``slow'' part of the biexponential?}

    %%%%
    % NEW STUFF
    {\color{red}
    \item{Find the percent error in $\EC$ at $\chi = 3$ for Adenine CCSD/cc-pVTZ. (Chao: Ec = 0.3526\%) [Done]}
    \item{Find the fraction of pair-points with interpair distances $< 3$ Bohr for Adenine CCSD/cc-pVTZ when $\chi = 3$  (Chao: p = 15.806\% when d $\leq$ 3) [Done]}
    \item{If we haven't done so already, we need to add molecular geometries and atomic basis sets to the SI. [Done! Chao: SI is ready with the optimized geometry]} 
    \item{We need to setup the public repo for energy-partitioning and WSS analysis. [Done]}
    \item{Add Figure of single grid point distance to nearest atom vs $\chi$. [Done]}
}

    %%%%
    % FINAL CLEANUP STUFF
    {\color{blue}
    \item{Add grant funding and whatnot. [Done]}
    \item{Finalize author ordering [Need to discuss with Dr. Matthews]} 
    \item{Format for specific journal}
    \item{Find specific reviewers. Probably Garnet Chan? }
    }
\end{enumerate}
\fi




\clearpage
\newpage
BLANK PAGE FOR MY SANITY
\newpage
